Fortune: Formula-Driven Reinforcement Learning for LLM Reasoning over Complex Tables

Tables are a fundamental medium for organizing and analyzing data, making table reasoning an essential capability for intelligent systems. Although large language models (LLMs) exhibit strong general reasoning abilities, they still struggle with accurate numerical reasoning over tabular data, particularly in complex table settings that require more than simple relational lookup. Spreadsheet formulas provide a powerful and expressive interface for executable symbolic operations, enabling sophisticated reasoning patterns that remain largely underexplored by existing LLMs. In this paper, we introduce Formula Tuning (Fortune), a formula-driven reinforcement learning (RL) framework that trains LLMs to generate executable spreadsheet formulas for question answering over tabular data, using execution success and answer correctness as reward signals. Building upon Fortune, we train Formula-R1 and evaluate its performance across seven table reasoning benchmarks, demonstrating competitive performance, particularly on tasks involving complex tables and multi-step numerical computation. Furthermore, Formula-R1-Plus, which integrates textual and formula-based reasoning, achieves further performance improvements. Beyond these empirical results, we provide insights into the roles of reinforcement learning and executable formula representations in table reasoning, highlighting the broader potential of symbolic RL to enhance the reasoning capabilities of LLMs.

==> tables/notation.tex <==
% Notation Table
\begin{table*}[h]
\caption{Notation used throughout the paper}
\label{tab:notation}
\begin{center}
\begin{tabular}{cl}
\toprule
\textbf{Notation} & \textbf{Description} \\
\midrule
\multicolumn{2}{l}{\textit{General}} \\
$s$ & Input instance, a pair $(\mathbb{T}, q)$ of table and question \\
$\mathbb{T}$ & Input table with $m$ rows and $n$ columns \\
$q$ & Natural-language query \\
$C_{i,j}$ & Cell at row $i$, column $j$ in the table \\
$m,n$ & Number of rows and columns in $\mathbb{T}$ \\
$a$ & Generated answer (textual or executed formula result) \\
$f$ & Spreadsheet formula generated by the model \\
$p(s)$ & Empirical distribution over table–query pairs \\
$r(a \mid s)$ & Reward function evaluating answer correctness \\
$a^\star(s)$ & Ground-truth answer for input $s$ \\
$\operatorname{exec}(f,\mathbb{T})$ & Deterministic executor applying $f$ to $\mathbb{T}$ \\
\midrule
\multicolumn{2}{l}{\textit{Policies}} \\
$\pi_\theta(a \mid s)$ & LM generation policy parameterized by $\theta$ \\
$\pi_\theta^{\mathrm{txt}}$ & Textual reasoning policy (free-text answer) \\
$\pi_\theta^{\mathrm{sym}}$ & Symbolic reasoning policy (formula-based) \\
$\pi_g$ & Teacher policy in supervised fine-tuning \\
$\pi_{\theta^\star}^{\mathrm{SFT}}$ & Optimal SFT policy under Assumption \\
$\pi_\theta^{\mathrm{RL}}$ & Policy learned via reinforcement learning \\
\midrule
\multicolumn{2}{l}{\textit{Objective and Metrics}} \\
$\mathbb{E}_{s\sim p,\,a\sim\pi}[\cdot]$ & Expectation under inputs and policy \\
$\mathbbm{1}[\cdot]$ & Indicator function (1 if true, 0 otherwise) \\
\midrule
\multicolumn{2}{l}{\textit{Assumptions and Events}} \\
$E_1$ & Event of selecting a correct high-level reasoning plan \\
$E_2$ & Event that all textual reasoning steps are correct \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

